Testing the Blazar Sequence with Spectra of Recently Discovered Dim Blazars from the Fermi Unassociated Catalog

Recent works have developed samples of blazars from among the Fermi-LAT unassociated sources via machine learning comparisons with known blazar samples. Continued analysis of these new blazars tests the predictions of the blazar sequence and enables more flux-complete samples of blazars as a population. Using Fermi, Swift, WISE, and archival radio data, we construct broadband spectral energy distributions for 106 recently identified blazars. Drawn from the unassociated 4FGL source sample, this new sample has a lower median flux than the overall sample of gamma-ray blazars. By measuring the synchrotron peak frequency, we compare our sample of new blazars with known blazars from the 4LAC catalog. We find that the bulk of the new blazars are similar to High-Synchrotron Peak (HSP) BL Lac objects, with a higher median synchrotron peak; the sample has a median $ log( {\nu}_{syn} /Hz ) = 15.5 $ via BLaST peak estimation, compared to $ log( {\nu}_{syn} /Hz ) = 14.2 $ for the 4LAC BL Lacs. Finally, we conduct synchrotron self-Compton (SSC) leptonic modeling, comparing fitted physical and phenomenological properties to brighter blazars. We find that the new blazars have smaller characteristic Lorentz factors ${\gamma}_{boost}$ and fitted magnetic fields $B$, in agreement with blazar sequence predictions. The new blazars have slightly higher Compton dominance ratios than expected, which may point to alternative emission models for these dim blazars. Our results extend the predictions of the blazar sequence to a sample of dimmer blazars, confirming the broad predictions of that theory.

==> 4FGL_blazar_SED(1)/tab_agnpy.tex <==
\begin{longrotatetable}
\begin{deluxetable*}{ccccccccccccc}% C for mathmode
\tablecaption{Synchrotron-self-Compton fits via agnpy with fixed $z = 0.34$ \label{tab:agnpyfits}}
\tablewidth{\columnwidth}
\tablehead{
\colhead{4FGL} & \colhead{XRT} & \colhead{$\log(k_e)$} & \colhead{$p_1$} & \colhead{$p_2$} & \colhead{$\log(\gamma_b)$} & \colhead{$\log(\gamma_{max})$} & \colhead{$\log(\gamma_{min})$} & \colhead{$\delta_D$} & \colhead{$\log(B)$} & \colhead{$\log(t_{var})$} & \colhead{$\chi^2_r$} \\
\colhead{} & \colhead{} & \colhead{} & \colhead{} & \colhead{} & \colhead{} & \colhead{} & \colhead{} & \colhead{} & \colhead{$\rm{G}$} & \colhead{$\rm{s}$} & \colhead{}
}
\startdata
J0004.4-4001 & J000434.1-400036 & -6.652 & 2.19 & 4.6 & 4.402 & 5.485 & 2.17 & 16.323 & -1.151 & 5.309 & 0.715 \\
J0025.4-4838 & J002536.8-483808 & -5.0 & 4.0 & 3.731 & 4.298 & 7.677 & 3.493 & 10.579 & -0.382 & 4.377 & 0.805 \\
J0026.1-0732 & J002611.9-073115 & -4.848 & 2.06 & 3.453 & 4.094 & 6.061 & 1.945 & 10.928 & -0.803 & 4.925 & 1.469 \\
J0031.5-5648 & J003135.1-564640 & -1.621 & -1.002 & 2.738 & 2.983 & 5.407 & 3.38 & 24.931 & -1.241 & 4.196 & 0.581 \\
J0037.2-2653 & J003729.6-265043 & -1.965 & -0.931 & 3.383 & 3.165 & 5.661 & 2.903 & 23.844 & -1.496 & 4.57 & 0.648 \\
J0057.9+6326 & J005758.1+632642 & -0.371 & -1.195 & 3.317 & 2.847 & 7.059 & 2.861 & 11.405 & -0.976 & 4.728 & 2.952 \\
J0058.3-4603 & J005806.4-460417 & -5.625 & 3.451 & 2.45 & 4.433 & 5.742 & 3.368 & 8.202 & -0.521 & 4.646 & 0.499 \\
J0118.3-6008 & J011823.10-600753 & -4.495 & 3.372 & 3.704 & 4.001 & 5.652 & 3.743 & 13.172 & -1.21 & 5.042 & 1.048 \\
J0120.2-7944 & J011914.7-794509 & -4.808 & 3.996 & 3.482 & 4.254 & 5.741 & 3.613 & 12.8 & -0.743 & 4.352 & 0.994 \\
J0125.9-6303 & J012548.3-630244 & -4.863 & 3.999 & 2.953 & 3.94 & 5.663 & 3.693 & 17.898 & -1.352 & 4.851 & 0.791 \\
J0156.3-2420 & J015624.4-242004 & -4.826 & -1.287 & 3.453 & 3.997 & 5.66 & 3.983 & 22.157 & -1.395 & 4.889 & 1.503 \\
J0159.0+3313 & J015905.0+331254 & -4.958 & 2.907 & 3.237 & 4.046 & 5.623 & 3.61 & 13.411 & -1.082 & 5.006 & 2.018 \\
J0209.8+2626 & J020946.5+262528 & -2.653 & 1.552 & 3.419 & 3.633 & 5.017 & 2.626 & 14.686 & -1.955 & 4.971 & 1.001 \\
J0231.0+3505 & J023112.4+350446 & -3.452 & 1.707 & 2.968 & 3.443 & 5.997 & 3.54 & 12.505 & -1.248 & 5.127 & 1.857 \\
J0240.2-0248 & J024004.6-024504 & -6.936 & 3.707 & 3.875 & 4.443 & 6.084 & 3.463 & 21.781 & -1.422 & 5.024 & 1.218 \\
J0259.0+0552 & J025857.4+055243 & -3.798 & 2.439 & 3.645 & 3.927 & 5.822 & 3.975 & 13.722 & -1.303 & 5.027 & 1.848 \\
J0301.6-5617 & J030115.2-561647 & -6.674 & 2.476 & 4.047 & 4.607 & 6.218 & 2.136 & 20.002 & -1.524 & 4.911 & 0.93 \\
J0302.5+3354 & J030226.7+335447 & -4.213 & 2.438 & 2.869 & 3.72 & 5.665 & 2.331 & 15.674 & -1.382 & 4.962 & 1.119 \\
J0327.6+2620 & J032737.2+262007 & -6.034 & 2.23 & 2.896 & 4.235 & 5.863 & 2.406 & 16.458 & -1.688 & 5.264 & 0.81 \\
J0406.2+0639 & J040607.7+063918 & -3.654 & 1.7 & 3.318 & 3.757 & 5.662 & 1.034 & 6.628 & -0.864 & 5.297 & 1.219 \\
J0409.2+2542 & J040921.6+254440 & -8.412 & 2.401 & 6.258 & 5.307 & 6.283 & 2.352 & 22.337 & -1.56 & 4.815 & 0.762 \\
J0427.8-6704 & J042749.5-670435 & -3.284 & 2.509 & 4.659 & 4.34 & 7.908 & 3.008 & 22.282 & -1.979 & 4.0 & 1.647 \\
J0537.5+0959 & J053745.9+095759 & -5.297 & 2.529 & 3.117 & 4.246 & 5.645 & 2.365 & 12.992 & -1.252 & 4.911 & 2.84 \\
J0539.2-6333 & J054002.9-633216 & -7.435 & 2.357 & 5.257 & 4.687 & 7.341 & 3.11 & 18.911 & -1.245 & 5.131 & 0.987 \\
J0610.8-4911 & J061031.8-491222 & -7.499 & -0.87 & 7.997 & 3.996 & 5.399 & 3.634 & 31.275 & -0.189 & 5.427 & 1.391 \\
J0610.8-4911 & J061100.0-491034 & -5.528 & 3.11 & 3.057 & 4.486 & 7.949 & 3.296 & 11.25 & -0.501 & 4.326 & 0.526 \\
J0620.7-5034 & J062045.7-503349 & -6.098 & 2.392 & 3.208 & 4.168 & 5.824 & 2.366 & 23.116 & -1.997 & 5.29 & 1.155 \\
J0633.9+5840 & J063400.1+584035 & -4.26 & 1.634 & 3.176 & 3.874 & 6.027 & 2.417 & 9.387 & -1.842 & 5.518 & 1.668 \\
J0650.6+2055 & J065035.4+205556 & -6.215 & 1.406 & 3.426 & 4.368 & 5.501 & 1.191 & 18.074 & -0.957 & 5.074 & 0.345 \\
J0704.3-4829 & J070421.8-482645 & -4.976 & 2.966 & 2.866 & 4.088 & 5.503 & 3.554 & 13.8 & -0.949 & 4.788 & 0.371 \\
J0738.6+1311 & J073843.4+131330 & -5.288 & 3.626 & 4.994 & 3.796 & 6.016 & 3.619 & 27.845 & -1.064 & 5.195 & 2.574 \\
J0800.1-5531 & J075949.3-553253 & -5.13 & 1.823 & 4.307 & 4.008 & 7.438 & 2.406 & 10.272 & -0.88 & 5.433 & 0.546 \\
J0800.1-5531 & J080013.1-553407 & -3.446 & 3.999 & 3.994 & 3.85 & 6.603 & 3.546 & 11.35 & -0.7 & 4.616 & 0.98 \\
J0800.9+0733 & J080056.5+073235 & -3.343 & 1.596 & 2.511 & 2.749 & 5.461 & 2.478 & 14.0 & -1.23 & 5.537 & 2.624 \\
J0838.5+4013 & J083902.8+401548 & -5.27 & 2.525 & 3.14 & 3.932 & 5.583 & 2.238 & 17.695 & -1.348 & 5.032 & 1.662 \\
J0903.5+4057 & J090342.8+405502 & -4.187 & 2.162 & 2.792 & 3.631 & 5.461 & 2.416 & 12.706 & -1.217 & 5.091 & 0.633 \\
J0906.1-1011 & J090616.2-101430 & -6.327 & 2.942 & 3.476 & 4.74 & 5.42 & 2.808 & 13.53 & -0.858 & 4.454 & 0.525 \\
J0910.1-1816 & J091003.9-181613 & -3.586 & 1.934 & 3.166 & 3.662 & 5.474 & 1.872 & 4.113 & -0.206 & 5.431 & 1.512 \\
J0914.5+6845 & J091429.10+684509 & -8.271 & 2.549 & 6.052 & 5.26 & 7.978 & 2.189 & 19.984 & -1.373 & 4.728 & 0.868 \\
J0928.4-5256 & J092818.7-525700 & -3.339 & 2.918 & 3.417 & 4.01 & 5.963 & 3.388 & 12.625 & -0.995 & 4.382 & 1.196 \\
J0930.9-3030 & J093058.0-303118 & -4.275 & 1.466 & 3.227 & 4.036 & 5.655 & 1.015 & 23.599 & -1.48 & 4.398 & 0.688 \\
J0934.5+7223 & J093334.0+722101 & -4.41 & 1.826 & 5.781 & 4.019 & 7.194 & 2.513 & 8.466 & -0.968 & 5.38 & 0.739 \\
J0938.8+5155 & J093835.0+515455 & -5.437 & 2.839 & 3.725 & 4.268 & 5.67 & 2.986 & 10.506 & -1.07 & 5.062 & 0.912 \\
J1008.2-1000 & J100749.3-094910 & -4.962 & 4.0 & 7.004 & 4.427 & 6.438 & 3.376 & 20.832 & -1.281 & 4.021 & 1.874 \\
J1008.2-1000 & J100802.5-095918 & -4.843 & 2.725 & 2.847 & 3.665 & 5.353 & 1.82 & 17.248 & -1.339 & 5.105 & 3.84 \\
J1008.2-1000 & J100848.6-095450 & -5.284 & 1.604 & 6.832 & 3.82 & 7.237 & 3.687 & 27.338 & -1.157 & 5.393 & 0.896 \\
J1011.1-4420 & J101132.0-442254 & -6.402 & 3.016 & 2.26 & 3.773 & 6.028 & 1.82 & 14.274 & -1.94 & 6.015 & 0.966 \\
J1016.1-4247 & J101620.8-424723 & -6.032 & 2.157 & 5.036 & 4.565 & 5.472 & 3.937 & 19.153 & -0.718 & 4.542 & 2.913 \\
J1018.1-2705 & J101750.2-270550 & -5.168 & 2.491 & 6.696 & 4.418 & 5.52 & 2.652 & 15.713 & -1.948 & 5.058 & 1.454 \\
J1018.1-4051 & J101801.5-405520 & -1.512 & 1.182 & 2.8 & 2.469 & 5.589 & 2.733 & 7.348 & -1.302 & 5.919 & 2.289 \\
J1018.1-4051 & J101807.6-404407 & -4.582 & 3.5 & 2.999 & 3.852 & 5.564 & 3.072 & 9.331 & -1.165 & 5.279 & 1.443 \\
J1024.5-4543 & J102432.6-454428 & -3.666 & 3.996 & 2.903 & 3.92 & 5.62 & 3.39 & 19.133 & -0.857 & 4.0 & 1.088 \\
J1034.7-4645 & J103438.7-464404 & -4.961 & 3.999 & 3.419 & 4.138 & 7.008 & 3.71 & 18.373 & -1.954 & 4.998 & 1.247 \\
J1048.4-5030 & J104824.2-502941 & -6.609 & 3.969 & 2.101 & 4.197 & 5.342 & 3.732 & 19.891 & -1.533 & 5.234 & 1.695 \\
J1049.8+2741 & J104938.8+274217 & -3.408 & 2.054 & 2.673 & 3.39 & 5.453 & 2.146 & 16.0 & -1.237 & 4.85 & 2.156 \\
J1106.7+3623 & J110636.7+362648 & -3.553 & 2.085 & 6.715 & 4.226 & 7.973 & 1.042 & 17.753 & -1.071 & 4.0 & 0.653 \\
J1111.4+0137 & J111114.2+013430 & -4.444 & 3.997 & 3.518 & 3.979 & 7.116 & 3.7 & 12.205 & -1.305 & 5.045 & 2.075 \\
J1119.9-1007 & J111948.2-100704 & -5.732 & 2.518 & 3.82 & 4.419 & 5.71 & 2.409 & 18.917 & -1.405 & 4.748 & 0.426 \\
J1122.0-0231 & J112213.8-022916 & -6.188 & 2.247 & 5.838 & 4.44 & 6.748 & 2.186 & 15.023 & -1.415 & 5.242 & 1.175 \\
J1146.0-0638 & J114600.8-063850 & -3.927 & 3.765 & 2.037 & 3.404 & 5.221 & 2.756 & 16.351 & -1.369 & 4.915 & 2.015 \\
J1155.2-1111 & J115514.7-111125 & -3.938 & 1.495 & 3.155 & 3.65 & 5.962 & 2.12 & 14.884 & -1.671 & 5.162 & 1.249 \\
J1220.1-2458 & J122014.5-245949 & -4.456 & 1.624 & 2.836 & 3.863 & 5.817 & 1.026 & 8.959 & -1.008 & 5.266 & 0.384 \\
J1243.7+1727 & J124351.6+172643 & -4.532 & 1.708 & 3.215 & 3.893 & 5.453 & 1.774 & 14.445 & -1.153 & 4.926 & 1.112 \\
J1256.8+5329 & J125630.4+533203 & -3.302 & 2.326 & 5.733 & 4.234 & 5.01 & 3.004 & 25.007 & -1.996 & 4.037 & 1.448 \\
J1326.0+3507 & J132544.4+350450 & -3.811 & 1.674 & 3.41 & 3.876 & 5.367 & 1.826 & 5.777 & -0.476 & 5.217 & 0.998 \\
J1326.0+3507 & J132622.3+350627 & -4.469 & 1.945 & 4.811 & 4.284 & 6.436 & 1.07 & 10.137 & -0.68 & 4.63 & 0.283 \\
J1415.9-1504 & J141546.1-150228 & -5.12 & 3.136 & 3.559 & 4.154 & 5.637 & 3.497 & 11.266 & -0.859 & 4.965 & 0.847 \\
J1429.8-0739 & J142949.7-073302 & -3.081 & 3.999 & 3.061 & 3.313 & 5.503 & 3.031 & 8.524 & -0.646 & 5.218 & 3.172 \\
J1513.0-3118 & J151244.8-311648 & -6.8 & 1.325 & 5.507 & 4.069 & 7.108 & 3.026 & 17.988 & -0.553 & 5.619 & 1.963 \\
J1514.8+4448 & J151450.10+444957 & -4.98 & 3.885 & 7.993 & 4.448 & 7.649 & 3.738 & 9.709 & -0.692 & 4.56 & 1.512 \\
J1528.4+2004 & J152835.10+200423 & -3.493 & 1.668 & 2.786 & 3.606 & 5.78 & 1.66 & 13.503 & -1.183 & 4.712 & 0.99 \\
J1545.0-6642 & J154459.0-664147 & -8.895 & 2.311 & 6.633 & 5.589 & 7.189 & 3.348 & 16.974 & -1.375 & 4.98 & 1.635 \\
J1557.2+3822 & J155711.9+382032 & -4.231 & 1.42 & 3.349 & 3.868 & 5.949 & 1.154 & 8.143 & -1.209 & 5.317 & 0.892 \\
J1631.8+4144 & J163146.7+414634 & -0.263 & -0.574 & 2.384 & 2.0 & 5.422 & 2.708 & 22.615 & -1.358 & 4.546 & 0.917 \\
J1637.5+3005 & J163728.2+300957 & -4.399 & 2.4 & 3.218 & 3.732 & 5.821 & 2.813 & 15.826 & -1.741 & 5.226 & 0.805 \\
J1637.5+3005 & J163739.3+301015 & -2.613 & 2.326 & 4.503 & 3.58 & 6.627 & 3.41 & 13.662 & -1.562 & 5.144 & 0.588 \\
J1644.8+1850 & J164457.3+185149 & -5.648 & 2.594 & 4.877 & 4.482 & 5.242 & 2.789 & 18.771 & -0.394 & 4.091 & 1.494 \\
J1645.0+1654 & J164500.0+165510 & -4.693 & 2.03 & 3.486 & 4.106 & 5.898 & 2.192 & 41.146 & -1.902 & 4.225 & 1.035 \\
J1651.7-7241 & J165151.5-724309 & -6.914 & 2.801 & 3.412 & 4.64 & 5.832 & 2.541 & 16.39 & -1.598 & 5.047 & 1.446 \\
J1720.6-5144 & J172032.7-514413 & -4.116 & 3.983 & 3.053 & 3.75 & 6.059 & 3.453 & 14.546 & -1.113 & 4.932 & 1.393 \\
J1818.5+2533 & J181830.9+253707 & -3.025 & -0.419 & 4.725 & 3.624 & 7.825 & 1.489 & 21.021 & -0.516 & 4.362 & 0.592 \\
J1846.9-0227 & J184650.7-022903 & -6.155 & 0.669 & 4.816 & 4.021 & 5.424 & 1.114 & 18.431 & -1.222 & 5.976 & 2.013 \\
J1910.8+2856 & J191052.2+285624 & -3.958 & 1.002 & 3.096 & 3.678 & 7.808 & 2.402 & 17.61 & -1.999 & 5.27 & 1.542 \\
J1910.8+2856 & J191059.4+285635 & -2.793 & 2.647 & 3.124 & 3.545 & 5.876 & 3.999 & 20.222 & -1.971 & 4.862 & 1.225 \\
J1918.0+0331 & J191803.6+033030 & -4.601 & 2.181 & 2.46 & 4.182 & 5.864 & 1.401 & 14.16 & -1.692 & 4.755 & 2.079 \\
J1927.5+0154 & J192731.3+015356 & -1.884 & -1.766 & 2.513 & 2.668 & 5.572 & 2.491 & 15.004 & -1.333 & 5.06 & 1.404 \\
J1955.3-5032 & J195512.5-503011 & -4.586 & 2.697 & 4.135 & 4.178 & 7.901 & 2.898 & 7.503 & -0.871 & 5.101 & 1.724 \\
J2008.4+1619 & J200827.6+161843 & -2.876 & 1.72 & 3.207 & 3.649 & 5.695 & 1.606 & 18.052 & -1.117 & 4.31 & 0.787 \\
J2041.1-6138 & J204111.10-613952 & -8.348 & 2.548 & 3.729 & 4.963 & 5.729 & 2.342 & 14.618 & -1.717 & 5.639 & 1.263 \\
J2046.9-5409 & J204700.5-541246 & -6.715 & 2.375 & 3.409 & 4.567 & 5.887 & 1.868 & 16.373 & -1.769 & 5.256 & 0.725 \\
J2109.6+3954 & J210936.4+395513 & -3.971 & 2.289 & 3.029 & 3.701 & 5.624 & 2.317 & 20.009 & -1.454 & 4.659 & 3.829 \\
J2114.9-3326 & J211452.0-332532 & -2.212 & 3.853 & 2.543 & 2.737 & 5.622 & 2.605 & 12.414 & -1.218 & 5.293 & 1.088 \\
J2159.6-4620 & J215935.9-461954 & -4.619 & 1.558 & 2.859 & 3.893 & 5.502 & 3.421 & 12.142 & -1.137 & 5.141 & 1.038 \\
J2207.1+2222 & J220704.3+222234 & -4.782 & 2.209 & 2.711 & 3.938 & 5.527 & 2.304 & 18.931 & -1.544 & 4.838 & 0.79 \\
J2222.9+1507 & J222253.9+151052 & -5.513 & 2.6 & 2.837 & 3.862 & 5.223 & 2.314 & 10.737 & -0.87 & 5.47 & 0.431 \\
J2225.8-0804 & J222552.9-080415 & -5.403 & 2.368 & 4.134 & 4.506 & 7.954 & 1.917 & 12.606 & -0.924 & 4.577 & 1.148 \\
J2237.2-6726 & J223709.3-672614 & -4.334 & 2.063 & 2.795 & 3.825 & 5.544 & 1.797 & 8.423 & -0.865 & 5.183 & 0.572 \\
J2240.3-5241 & J224017.5-524117 & -6.465 & 2.348 & 4.262 & 4.598 & 5.399 & 2.183 & 15.088 & -1.169 & 5.055 & 0.757 \\
J2247.7-5857 & J224744.10-585500 & -2.493 & 2.02 & 2.953 & 3.228 & 5.703 & 2.568 & 7.819 & -1.047 & 5.29 & 1.75 \\
J2303.9+5554 & J230351.7+555618 & -3.744 & 2.701 & 2.64 & 3.351 & 6.187 & 2.924 & 15.126 & -2.0 & 5.437 & 2.605 \\
J2311.6-4427 & J231145.6-443220 & -4.441 & 2.21 & 3.819 & 4.023 & 5.553 & 3.6 & 10.379 & -0.815 & 4.93 & 0.82 \\
J2317.7+2839 & J231740.0+283954 & -6.031 & 3.165 & 1.377 & 4.071 & 5.1 & 2.768 & 21.651 & -1.284 & 4.82 & 0.725 \\
J2326.9-4130 & J232653.2-412713 & -4.842 & 2.334 & 4.902 & 3.998 & 7.708 & 2.485 & 7.891 & 0.158 & 5.0 & 0.608 \\
J2336.9-8427 & J233627.1-842648 & -6.009 & 3.76 & 2.174 & 4.586 & 5.317 & 3.478 & 10.276 & -0.48 & 4.391 & 0.446 \\
J2337.7-2903 & J233730.2-290240 & -0.815 & 2.583 & 2.611 & 2.375 & 5.141 & 2.087 & 8.092 & -0.346 & 5.041 & 0.696 \\
J2351.4-2818 & J235136.5-282154 & -6.182 & 2.059 & 4.489 & 4.059 & 5.468 & 2.12 & 21.662 & -1.009 & 5.258 & 1.079 \\
\enddata
\end{deluxetable*}
\end{longrotatetable}

==> 4FGL_blazar_SED(1)/tab_initials.tex <==
\startlongtable
\begin{deluxetable}{cccc}% C for mathmode
\tablecaption{SSC parameter initialization and ranges for agnpy fitting.}
\tablewidth{\columnwidth}
\label{tab:initial}
\tablehead{
\colhead{Parameter} & \colhead{lower} & \colhead{initial} & \colhead{upper} 
}
\startdata
\hline
$\log (k_e)$ & -12 & -4 & 0 \\
$p_1$ & -2 & 2.5 & 4 \\
$p_2$ & 1 & 4 & 8 \\
$\log (\gamma_b)$ & 2 & 5 & 6 \\
$\log (\gamma_{min})$ & 1 & 2 & 4 \\
$\log (\gamma_{max})$ & 5 & 6 & 8 \\
\hline
$z$ \textbf{(fixed)} & & $0.34$ & \\
$\delta_D$ & 1 & 20 & 100 \\
$\log (B/\rm{G})$ & -2 & -1 & 1 \\
$\log (t_{var}/\rm{s})$ & 4 & 5 & 8 \\
\enddata
\end{deluxetable}

==> 4FGL_blazar_SED(1)/tab_phenom.tex <==
\begin{longrotatetable}
\begin{deluxetable*}{cccccccccc}% C for mathmode
\tablecaption{Phenomological features of the broadband SEDs from agnpy fitting unless otherwise noted \label{tab:phenom}}
\tablewidth{\columnwidth}
\tablehead{
\colhead{4FGL} & \colhead{XRT} & \colhead{$\log(\nu_{syn,BLAST}$)} & \colhead{$\log(\delta \nu_{syn,BLAST})$} & \colhead{$\log(\nu_{syn})$} & \colhead{$\log(\nu F_{\nu,syn})$} & \colhead{$\log(\nu_{Com})$} & \colhead{$\log(\nu F_{\nu,Com})$} & \colhead{$\log(F_{bol})$} \\
\colhead{} & \colhead{} & \colhead{$\log(\rm{Hz})$} & \colhead{$\log(\rm{Hz})$} & \colhead{$\log(\rm{Hz})$} & \colhead{$\log(\rm{erg/s/cm^2})$} & \colhead{$\log(\rm{Hz})$} & \colhead{$\log(\rm{erg/s/cm^2})$} & \colhead{$\log(\rm{erg/s/cm^2})$}
}
\startdata
J0004.4-4001 & J000434.1-400036 & 14.707 & 0.626 & 15.191 & -11.728 & 23.7 & -12.423 & -9.545 \\
J0025.4-4838 & J002536.8-483808 & 15.794 & 1.326 & 14.571 & -12.304 & 22.519 & -12.238 & -9.931 \\
J0026.1-0732 & J002611.9-073115 & 16.6 & 0.829 & 15.051 & -12.444 & 23.84 & -12.654 & -10.01 \\
J0031.5-5648 & J003135.1-564640 & 15.595 & 1.047 & 16.633 & -12.51 & 24.601 & -12.615 & -10.058 \\
J0037.2-2653 & J003729.6-265043 & 13.787 & 1.759 & 13.089 & -12.449 & 21.297 & -12.633 & -9.975 \\
J0057.9+6326 & J005758.1+632642 & 15.678 & 0.708 & 12.889 & -12.545 & 21.197 & -12.237 & -9.693 \\
J0058.3-4603 & J005806.4-460417 & 17.091 & 0.821 & 17.734 & -12.773 & 24.801 & -12.839 & -10.215 \\
J0118.3-6008 & J011823.10-600753 & 14.24 & 1.155 & 14.411 & -12.248 & 23.119 & -12.325 & -9.916 \\
J0120.2-7944 & J011914.7-794509 & 15.861 & 1.318 & 14.451 & -12.586 & 22.679 & -12.524 & -10.171 \\
J0125.9-6303 & J012548.3-630244 & 16.073 & 0.771 & 16.312 & -12.599 & 24.401 & -12.817 & -10.123 \\
J0156.3-2420 & J015624.4-242004 & 15.712 & 0.712 & 14.951 & -11.923 & 24.521 & -12.346 & -9.708 \\
J0159.0+3313 & J015905.0+331254 & 15.737 & 0.838 & 14.491 & -12.324 & 24.04 & -12.511 & -9.903 \\
J0209.8+2626 & J020946.5+262528 & 16.719 & 1.143 & 13.209 & -12.906 & 21.518 & -12.123 & -9.795 \\
J0231.0+3505 & J023112.4+350446 & 16.664 & 0.933 & 16.853 & -12.721 & 24.381 & -12.901 & -10.171 \\
J0240.2-0248 & J024004.6-024504 & 14.822 & 0.649 & 13.81 & -11.782 & 21.938 & -12.247 & -9.597 \\
J0259.0+0552 & J025857.4+055243 & 15.377 & 0.625 & 14.791 & -12.062 & 24.04 & -11.873 & -9.598 \\
J0301.6-5617 & J030115.2-561647 & 14.554 & 1.913 & 15.291 & -12.401 & 23.94 & -12.664 & -9.962 \\
J0302.5+3354 & J030226.7+335447 & 15.73 & 0.813 & 16.653 & -12.605 & 23.78 & -12.675 & -9.99 \\
J0327.6+2620 & J032737.2+262007 & 15.973 & 0.772 & 16.593 & -12.521 & 24.741 & -12.732 & -10.018 \\
J0406.2+0639 & J040607.7+063918 & 15.405 & 1.295 & 14.23 & -12.773 & 22.959 & -12.575 & -10.107 \\
J0409.2+2542 & J040921.6+254440 & 15.734 & 0.889 & 16.513 & -12.129 & 25.101 & -12.467 & -9.803 \\
J0427.8-6704 & J042749.5-670435 & 15.044 & 2.093 & 14.23 & -13.143 & 22.338 & -11.696 & -9.422 \\
J0537.5+0959 & J053745.9+095759 & 15.583 & 0.957 & 15.111 & -12.786 & 23.96 & -12.697 & -10.096 \\
J0539.2-6333 & J054002.9-633216 & 14.192 & 1.023 & 15.592 & -11.928 & 24.361 & -12.686 & -9.758 \\
J0610.8-4911 & J061031.8-491222 & 14.529 & 0.557 & 15.792 & -9.862 & 23.98 & -12.752 & -8.073 \\
J0610.8-4911 & J061100.0-491034 & 16.655 & 1.273 & 14.35 & -12.874 & 23.84 & -12.861 & -10.134 \\
J0620.7-5034 & J062045.7-503349 & 15.348 & 0.615 & 14.391 & -12.439 & 23.56 & -12.756 & -9.939 \\
J0633.9+5840 & J063400.1+584035 & 14.913 & 1.062 & 13.75 & -13.233 & 23.72 & -12.796 & -10.34 \\
J0650.6+2055 & J065035.4+205556 & 16.411 & 1.055 & 15.772 & -11.331 & 24.741 & -11.912 & -9.148 \\
J0704.3-4829 & J070421.8-482645 & 16.177 & 0.871 & 16.693 & -12.376 & 24.461 & -12.518 & -9.914 \\
J0738.6+1311 & J073843.4+131330 & 14.496 & 0.517 & 14.491 & -10.78 & 22.499 & -12.031 & -8.916 \\
J0800.1-5531 & J075949.3-553253 & 13.891 & 1.17 & 14.591 & -11.896 & 22.739 & -12.353 & -9.694 \\
J0800.1-5531 & J080013.1-553407 & 13.636 & 1.808 & 14.371 & -12.287 & 22.439 & -12.235 & -9.934 \\
J0800.9+0733 & J080056.5+073235 & 15.365 & 0.779 & 16.653 & -12.037 & 24.701 & -13.152 & -9.849 \\
J0838.5+4013 & J083902.8+401548 & 15.142 & 0.782 & 14.491 & -12.593 & 23.239 & -13.089 & -10.111 \\
J0903.5+4057 & J090342.8+405502 & 14.977 & 0.846 & 16.373 & -12.683 & 24.0 & -12.97 & -10.228 \\
J0906.1-1011 & J090616.2-101430 & 14.9 & 1.836 & 15.552 & -12.787 & 22.999 & -12.516 & -9.981 \\
J0910.1-1816 & J091003.9-181613 & 15.853 & 0.986 & 14.571 & -12.69 & 23.039 & -12.69 & -10.113 \\
J0914.5+6845 & J091429.10+684509 & 15.799 & 0.923 & 16.493 & -12.321 & 24.601 & -12.624 & -9.91 \\
J0928.4-5256 & J092818.7-525700 & 15.527 & 1.159 & 14.21 & -12.696 & 23.099 & -12.021 & -9.696 \\
J0930.9-3030 & J093058.0-303118 & 15.79 & 0.774 & 14.811 & -12.609 & 24.14 & -12.527 & -10.051 \\
J0934.5+7223 & J093334.0+722101 & 13.994 & 1.475 & 14.31 & -12.127 & 22.238 & -12.077 & -9.744 \\
J0938.8+5155 & J093835.0+515455 & 13.151 & 1.428 & 14.511 & -12.712 & 22.459 & -12.655 & -10.102 \\
J1008.2-1000 & J100749.3-094910 & 13.157 & 1.224 & 13.73 & -12.439 & 21.518 & -11.767 & -9.632 \\
J1008.2-1000 & J100802.5-095918 & 12.278 & 0.672 & 16.152 & -12.596 & 23.239 & -13.251 & -10.128 \\
J1008.2-1000 & J100848.6-095450 & 13.842 & 0.921 & 14.451 & -10.533 & 22.459 & -11.726 & -8.724 \\
J1011.1-4420 & J101132.0-442254 & 17.268 & 0.773 & 17.273 & -11.651 & 25.822 & -12.627 & -9.484 \\
J1016.1-4247 & J101620.8-424723 & 15.577 & 0.617 & 15.972 & -11.587 & 24.701 & -12.075 & -9.519 \\
J1018.1-2705 & J101750.2-270550 & 15.534 & 1.811 & 14.13 & -12.655 & 22.118 & -12.023 & -9.672 \\
J1018.1-4051 & J101801.5-405520 & 13.584 & 1.911 & 16.352 & -12.594 & 23.36 & -12.798 & -10.061 \\
J1018.1-4051 & J101807.6-404407 & 13.452 & 2.088 & 12.949 & -12.732 & 23.179 & -12.719 & -10.106 \\
J1024.5-4543 & J102432.6-454428 & 16.675 & 0.985 & 16.993 & -12.767 & 24.12 & -12.494 & -9.985 \\
J1034.7-4645 & J103438.7-464404 & 16.472 & 0.91 & 13.67 & -12.701 & 22.759 & -12.537 & -10.088 \\
J1048.4-5030 & J104824.2-502941 & 15.068 & 0.656 & 16.433 & -11.817 & 25.021 & -12.53 & -9.679 \\
J1049.8+2741 & J104938.8+274217 & 15.567 & 0.756 & 16.593 & -12.44 & 24.2 & -12.701 & -10.005 \\
J1106.7+3623 & J110636.7+362648 & 12.819 & 1.301 & 14.831 & -12.732 & 22.979 & -12.235 & -9.964 \\
J1111.4+0137 & J111114.2+013430 & 16.401 & 1.622 & 14.15 & -12.606 & 23.039 & -12.646 & -10.179 \\
J1119.9-1007 & J111948.2-100704 & 15.428 & 0.701 & 15.031 & -12.428 & 23.42 & -12.434 & -9.85 \\
J1122.0-0231 & J112213.8-022916 & 15.625 & 0.82 & 14.831 & -12.156 & 23.259 & -12.408 & -9.832 \\
J1146.0-0638 & J114600.8-063850 & 16.06 & 0.875 & 16.292 & -12.033 & 25.201 & -12.195 & -9.731 \\
J1155.2-1111 & J115514.7-111125 & 15.624 & 0.728 & 13.69 & -12.906 & 23.58 & -12.936 & -10.284 \\
J1220.1-2458 & J122014.5-245949 & 16.661 & 0.976 & 17.073 & -12.416 & 24.3 & -12.433 & -9.87 \\
J1243.7+1727 & J124351.6+172643 & 15.236 & 0.622 & 14.611 & -12.544 & 23.66 & -12.801 & -10.126 \\
J1256.8+5329 & J125630.4+533203 & 13.797 & 2.319 & 14.03 & -13.105 & 22.058 & -12.034 & -9.816 \\
J1326.0+3507 & J132544.4+350450 & 14.81 & 0.999 & 14.751 & -12.474 & 23.279 & -12.305 & -9.902 \\
J1326.0+3507 & J132622.3+350627 & 14.219 & 2.325 & 15.251 & -12.473 & 23.8 & -12.319 & -9.989 \\
J1415.9-1504 & J141546.1-150228 & 15.109 & 1.199 & 14.35 & -12.315 & 23.099 & -12.478 & -9.94 \\
J1429.8-0739 & J142949.7-073302 & 14.268 & 1.069 & 13.349 & -12.446 & 23.139 & -12.708 & -9.931 \\
J1513.0-3118 & J151244.8-311648 & 14.417 & 0.588 & 15.251 & -10.565 & 23.44 & -12.269 & -8.635 \\
J1514.8+4448 & J151450.10+444957 & 14.531 & 1.852 & 14.711 & -12.316 & 23.119 & -11.8 & -9.728 \\
J1528.4+2004 & J152835.10+200423 & 16.477 & 1.002 & 17.073 & -12.868 & 24.461 & -12.92 & -10.319 \\
J1545.0-6642 & J154459.0-664147 & 16.923 & 0.941 & 17.173 & -11.756 & 25.442 & -12.084 & -9.493 \\
J1557.2+3822 & J155711.9+382032 & 15.668 & 0.778 & 14.21 & -13.033 & 23.239 & -13.012 & -10.488 \\
J1631.8+4144 & J163146.7+414634 & 15.875 & 0.867 & 16.713 & -12.233 & 25.221 & -12.648 & -9.961 \\
J1637.5+3005 & J163728.2+300957 & 13.168 & 1.453 & 13.61 & -12.884 & 22.839 & -13.03 & -10.308 \\
J1637.5+3005 & J163739.3+301015 & 13.39 & 0.968 & 13.289 & -12.06 & 20.937 & -11.607 & -9.482 \\
J1644.8+1850 & J164457.3+185149 & 14.713 & 1.026 & 15.932 & -12.152 & 23.74 & -12.632 & -9.843 \\
J1645.0+1654 & J164500.0+165510 & 15.751 & 0.793 & 14.531 & -12.524 & 23.44 & -12.632 & -10.031 \\
J1651.7-7241 & J165151.5-724309 & 14.62 & 1.34 & 15.151 & -12.814 & 23.079 & -12.846 & -10.141 \\
J1720.6-5144 & J172032.7-514413 & 16.751 & 0.938 & 14.01 & -12.34 & 24.12 & -12.443 & -9.766 \\
J1818.5+2533 & J181830.9+253707 & 14.042 & 0.809 & 14.671 & -11.372 & 22.358 & -11.864 & -9.327 \\
J1846.9-0227 & J184650.7-022903 & 14.29 & 0.455 & 14.631 & -10.252 & 22.959 & -11.081 & -8.262 \\
J1910.8+2856 & J191052.2+285624 & 16.243 & 0.938 & 13.61 & -12.646 & 23.9 & -12.356 & -9.751 \\
J1910.8+2856 & J191059.4+285635 & 15.686 & 0.888 & 14.491 & -12.703 & 24.601 & -12.261 & -9.941 \\
J1918.0+0331 & J191803.6+033030 & 15.64 & 0.88 & 17.113 & -12.641 & 25.281 & -12.199 & -9.867 \\
J1927.5+0154 & J192731.3+015356 & 15.859 & 0.729 & 16.813 & -12.155 & 24.781 & -12.454 & -9.782 \\
J1955.3-5032 & J195512.5-503011 & 15.885 & 1.212 & 14.471 & -12.678 & 22.178 & -12.267 & -9.875 \\
J2008.4+1619 & J200827.6+161843 & 15.952 & 1.637 & 14.27 & -12.715 & 23.339 & -12.513 & -9.995 \\
J2041.1-6138 & J204111.10-613952 & 15.262 & 0.732 & 15.712 & -12.139 & 24.24 & -12.433 & -9.698 \\
J2046.9-5409 & J204700.5-541246 & 15.239 & 1.461 & 15.131 & -12.586 & 24.28 & -12.681 & -10.058 \\
J2109.6+3954 & J210936.4+395513 & 15.81 & 0.744 & 14.19 & -12.945 & 24.32 & -12.879 & -10.276 \\
J2114.9-3326 & J211452.0-332532 & 16.192 & 1.054 & 16.913 & -12.011 & 24.621 & -12.372 & -9.648 \\
J2159.6-4620 & J215935.9-461954 & 15.54 & 0.758 & 16.393 & -12.285 & 24.421 & -12.354 & -9.819 \\
J2207.1+2222 & J220704.3+222234 & 15.346 & 0.627 & 16.473 & -12.51 & 24.481 & -12.621 & -10.024 \\
J2222.9+1507 & J222253.9+151052 & 14.957 & 0.89 & 16.172 & -12.133 & 23.38 & -12.823 & -9.749 \\
J2225.8-0804 & J222552.9-080415 & 15.472 & 1.036 & 15.512 & -12.651 & 24.04 & -12.566 & -10.077 \\
J2237.2-6726 & J223709.3-672614 & 16.106 & 0.784 & 16.773 & -12.537 & 24.22 & -12.62 & -10.019 \\
J2240.3-5241 & J224017.5-524117 & 15.002 & 0.73 & 15.512 & -11.957 & 24.2 & -12.129 & -9.548 \\
J2247.7-5857 & J224744.10-585500 & 15.508 & 1.453 & 16.413 & -12.92 & 23.139 & -12.642 & -10.082 \\
J2303.9+5554 & J230351.7+555618 & 16.605 & 0.8 & 17.353 & -12.483 & 24.781 & -12.558 & -9.951 \\
J2311.6-4427 & J231145.6-443220 & 15.104 & 1.693 & 14.711 & -12.448 & 23.279 & -12.618 & -10.161 \\
J2317.7+2839 & J231740.0+283954 & 15.152 & 0.556 & 16.373 & -11.613 & 25.502 & -12.201 & -9.519 \\
J2326.9-4130 & J232653.2-412713 & 13.578 & 1.096 & 18.294 & -13.669 & 22.819 & -12.335 & -9.453 \\
J2336.9-8427 & J233627.1-842648 & 16.124 & 0.918 & 17.173 & -12.867 & 23.84 & -12.607 & -10.061 \\
J2337.7-2903 & J233730.2-290240 & 15.841 & 0.768 & 16.673 & -12.22 & 23.98 & -12.747 & -9.871 \\
J2351.4-2818 & J235136.5-282154 & 14.196 & 0.587 & 14.811 & -11.302 & 22.899 & -12.485 & -9.208 \\
\enddata
\end{deluxetable*}
\end{longrotatetable}
